Average motion of emerging solar active region polarities I: Two phases of emergence

Our goal is to constrain models of active region formation by tracking the average motion of active region polarity pairs as they emerge onto the surface. We measured the motion of the two main opposite polarities in 153 emerging active regions (EARs) using line-of-sight magnetic field observations from the Solar Dynamics Observatory Helioseismic Emerging Active Region (SDO/HEAR) survey (Schunker et al. 2016). We first measured the position of each of the polarities eight hours after emergence and tracked their location forwards and backwards in time. We find that, on average, the polarities emerge with an east-west orientation and the separation speed between the polarities increases. At about 0.1 days after emergence, the average separation speed reaches a peak value of 229 +/- 11 m/s, and then starts to decrease, and about 2.5 days after emergence the polarities stop separating. We also find that the separation and the separation speed in the east-west direction are systematically larger for active regions with higher flux. Our results reveal two phases of the emergence process defined by the rate of change of the separation speed as the polarities move apart. Phase 1 begins when the opposite polarity pairs first appear at the surface, with an east-west alignment and an increasing separation speed. We define Phase 2 to begin when the separation speed starts to decrease, and ends when the polarities have stopped separating. This is consistent with the picture of Chen, Rempel, & Fan (2017): the peak of a flux tube breaks through the surface during Phase 1. During Phase 2 the magnetic field lines are straightened by magnetic tension, so that the polarities continue to move apart, until they eventually lie directly above their anchored subsurface footpoints.

==> measure_area_obs_unc_table_AR11158_TI+02.tex <==
\begin{tabular}{l || c | c | c | c  }
    & $x_f$ & $y_f$ & $x_l$ & $y_l$ \\ 
    & [pix] & [pix] & [pix] & [pix] \\ 
\hline
 ave0   & 246.5287 & 256.1639 & 278.8013 & 253.9687 \\ 
 ave1   & 246.5272 & 256.1652 & 278.8108 & 253.9677 \\ 
 ave2   & 246.5236 & 256.1654 & 278.8177 & 253.9663 \\ 
 ave3   & 246.5215 & 256.1635 & 278.8251 & 253.9673 \\ 
 \hline  
 $\sigma$ &    0.003 &    0.001 &    0.010 &    0.001 \\ 
\end{tabular}

